Where Do You Want To Invest? Predicting Startup Funding From Freely, Publicly Available Web Information

We consider in this paper the problem of predicting the ability of a startup to attract investments using freely, publicly available data. Information about startups on the web usually comes either as unstructured data from news, social networks, and websites or as structured data from commercial databases, such as Crunchbase. The possibility of predicting the success of a startup from structured databases has been studied in the literature and it has been shown that initial public offerings (IPOs), mergers and acquisitions (M\&A) as well as funding events can be predicted with various machine learning techniques. In such studies, heterogeneous information from the web and social networks is usually used as a complement to the information coming from databases. However, building and maintaining such databases demands tremendous human effort. We thus study here whether one can solely rely on readily available sources of information, such as the website of a startup, its social media activity as well as its presence on the web, to predict its funding events. As illustrated in our experiments, the method we propose yields results comparable to the ones making also use of structured data available in private databases.

==> Framework.tex <==
\section{Data Collection}\label{sec:data}


\subsection{Features}

In this section we describe strartup features that we extracted from web for the purpose of startup success prediction. They can be split into the following categories. 

\subsubsection{Social networks presence features}
Over the last two decades the impact of social networks on different social, economic and political processes became remarkable. For a startup it might be crucial to reach the potential audience via social media. \cite{zhang2017predicting} study highlights importance of social media presence for a crowdfunding success campaign of a startup. Therefore in our work we analyse social media activity of startups and extract various features in order to predict the funding success. 

The first set of binary social media presence features indicates whether a startup has an account in several popular social medias:
\begin{itemize}
	\item Facebook
	\item Instagram
	\item Linkedin
	\item YouTube
	\item Twitter
	\item Blog on the startup own website
\end{itemize}
This information is extracted with simple script that searches for social network buttons on a website of a startup. 

The largest fraction of the features in our dataset comes from Twitter. It is remarkable that given a list of startups accounts names one can extract twitter features using Twitter api \footnote{\url{https://developer.twitter.com}}  in a very straightforward manner, since Twitter api is freely available to everyone. The only limitation is that one can extract only the last 2300 tweets of a certain user. However according to our observations most startups tend to have far less tweets in their lifetime. Thus for many startups it is possible to analyze lifetime activity on Twitter. In our work however we focus on analysis of twitter activity during one year that precedes the year for which we try to predict funding events. 

In principle great variety of features can be extracted from the records about user's activity. In our work we propose the following set of features:
\begin{itemize}
	\item aggregated monthly startup's twitter account statistics for the last year such as: number of posted tweets, mean/max number of likes and retweets of user's tweets; modal language of user tweets. The same tweets statistics are collected for a set of tweets that \textit{mention} the startup's twitter account and for the tweets that are \textit{retweeted} by a startup's twitter account.
	\item information about \textit{hashtags} utilized by startups. For 500 hashtags most frequent among different startups the information about total amount of tweets with each hashtag is stored.
\end{itemize}

\subsubsection{Professional events attendance features}
Complimentary to the information about a startup activity in social media could be information about its offline social activity, such as attendance of scientific and industrial conferences, workshops, pitches, summits etc. Such events allow startups to form professional connections as well as draw attention of potential investors and customers. A formal definition of a startup event however is hard to 


\subsubsection{Tags}\label{tags}
Analysis of website allows us to assign on of 200(?) tags to each startup \todo{Hamid: please describe how the tags are extracted}

Examples of tags are: \textit{AI, biotech, blockchain, tourism} etc. Full list of possible tags can be found in appendix.

\subsubsection{Patents statistics}

\todo{Hamid: how we extract patents information}

Apparently we exclude from analysis the patents that were registered after the date $t$ from which we want to predict funding events.

In principle it is possible to extract various features from patents. In our work however we only use the following statistics about patents:
\begin{itemize}
	\item total number of patents
	\item minimal and average age of patents
\end{itemize}

\subsubsection{Google search results features}
In \cite{sharchilev2018web} the authors have shown that an extremely useful set of features for the task of startup success prediction can be extracted from crawl of the observable web for the startups presence. For the purpose of extraction of these features the authors analyze the data used in building of Yandex\footnote{\url{https://yandex.ru}}, a major Russian search engine. For each startup they count number of references to the startup's website on the web-pages from different domains. Unfortunately, not everyone is as lucky to have a web index information at hand. 

In our study we try to extract similar information using more widely available tools, in particular Google search API\footnote{\url{https://developers.google.com/custom-search/v1/overview}}. For each startup we analyze search results with a date within a year preceding the start of \textit{prediction period}. For each startup name and a date range we make a query, filter irrelevant results and perform the analysis of domains frequencies similar to \cite{sharchilev2018web}. In order to exclude irrelevant results we check whether snippet of a search result contains the startup's name. Since the purpose of this work is to build model with free tools only we constrain ourselves to the amount of queries available with The Google Cloud Platform Free Tier \footnote{\url{https://cloud.google.com/free/docs/gcp-free-tier}}. Therefore we obtain only top 10 results for a given startup name and a date range. The following statistics are then extracted:

\begin{itemize}
	\item number of relevant results. We assume that result is related to startup only if a snippet of result contains the startup's name.
	\item total number of results as reported by Google
	\item number of results on each of 500 domains most often referred 
\end{itemize}

\subsubsection{Other features}

\begin{itemize}
	
	\item binary for startup receiving funding on the year preceding the year for which the forecasts are made. Information about the previous year funding is extracted in the same fashion as described in section \ref{subsec:fundingextraction}. Due to the online fashion of our algorithm and the fact that we were adding new sources for analysis incrementally information about old funding events is very incomplete.
	\item number of people listed on team/people page of a startup website; number of people that give reference to their Linkedin account.
\end{itemize}



==> Problem.tex <==
\section{Problem Statement}\label{sec:problem}

Following \cite{sharchilev2018web} we set out to predict \textit{funding} events. More precisely we want to predict whether a startup will secure funding round in a given amount of time (\textit{horizon}). However our task is significantly more difficult. Since we use data purely automatically extracted from web, we do not in most cases have information concerning the type of funding round. Also most of the funding events collected by our system took place during the last year, therefore we cannot as \cite{sharchilev2018web} put it "filter stale startups" by making predictions only for the startups that received seed funding during the last year.

Intended use-case of the model is investment decision-making process, therefore the investor-centric approach is adopted: for a fixed date $t$ predictions for each candidate startup are made.

For the purpose of data augmentation several dates $t$ are chosen. Thus for each startup forecasts are made at different moments. For every train/test split however each startup occurs either only in train set or in test set.


